Configurational Forces in Penetration Processes

With a loose reference to problems of penetration in biomechanics (for instance, a nanoparticle penetrating through a cell's membrane or a cell sucked with a pipette), the role of configurational forces is investigated during the process in which a compliant intruder is inserted into an elastic structure. For insertion into a rigid constraint, a configurational force proportional to the square of the strain needed to deform the body, which is penetrating, is found. This force has a more complex structure when the compliance of the constraint is kept into account, but in all cases, it tends to expel the penetrating body.

==> referenc.tex <==
%\clearpage
\begin{thebibliography}{}

\bibitem{bigoni_libro} Bigoni, D. (2012) Nonlinear solid mechanics. Cambridge University Press.

\bibitem{conf1} D. Bigoni, F. Dal Corso, F. Bosi and D. Misseroni (2015) Eshelby-like forces acting on elastic structures: theoretical and experimental proof. Mechanics of Materials, 80, 368-374.

\bibitem{conf4} D. Bigoni, F. Bosi, F. Dal Corso and D. Misseroni (2014) Instability of a penetrating blade. Journal of the Mechanics and Physics of Solids, 64, 411-425

\bibitem{conf2} D. Bigoni, F. Dal Corso, D.Misseroni and F. Bosi (2014) Torsional locomotion. Proceedings of the Royal Society A, 20140599.

\bibitem{conf3} Bosi, F., Misseroni, D., Dal Corso, F. and Bigoni, D. (2015) Self-encapsulation, or the \lq dripping' of an elastic rod. Proceedings of the Royal Society A, 471, 20150195.

\bibitem{boal} Boal, D. (2002) Mechanics of the cell. Cambridge University Press. 

\bibitem{menzel} Daddi-Moussa-Ider, A., Goh, S., Liebchen, B., Hoell, C., Mathijssen, Arnold J.T.M., Guzm\'n-Lastra, F., Scholz, C., Menzel, A.M., L\"owen, H. (2019) Membrane penetration and trapping of an active particle. J. Chem. Phys. 150, 064906. 

\bibitem{deseri1} L. Deseri, P. Pollaci, M. Zingales, K. Dayal (2016) Fractional hereditariness of lipid membranes: instabilities and linearized evolution. J. Mech. Behaviour Biomed. Materials 58, 11-27. 

\bibitem{deseri2} L. Deseri, G. Zurlo (2013) The stretching elasticity of biomembranes determines their line tension and bending rigidity, Biomech. Modeling Mechanobiology 12 1233-1242. 

\bibitem{disher} Discher, D.E., Mohandas, N., Evans E.A. (1994) Molecular maps of red cell deformation: hidden elasticity and in situ connectivity. Science, 266, 1032-1035.

\bibitem{disher2} Discher, D.E., Boal, D.H., Boey, S.K. (1998) Simulations of the erythrocyte cytoskeleton at large deformation - II. micropipette aspiration. Biophys. J.  75, Issue 3, 1584-1597.

\bibitem{eshelby}  Eshelby, J.D. (1951) The force on an elastic singularity. Phil. Trans. Roy. Soc. London A 244, 87-112.

\bibitem{holz4} G Franceschini, D Bigoni, P Regitnig, GA Holzapfel (2006) Brain tissue deforms similarly to filled elastomers and follows consolidation theory J. Mech. Phys. Solids 54, 2592-2620. 


\bibitem{holz2} GA Holzapfel, TC Gasser, RW Ogden (2000) A new constitutive framework for arterial wall mechanics and a comparative study of material models Journal of elasticity and the physical science of solids 61, 1-48. 

\bibitem{holz3} GA Holzapfel, G Sommer, P Regitnig (2004) Anisotropic mechanical properties of tissue components in human atherosclerotic plaques. J. Biomech. Eng. 126, 657-665. 

\bibitem{holz5} LA Mihai, S Budday, GA Holzapfel, E Kuhl, A Goriely (2017) A family of hyperelastic models for human brain tissue J. Mech. Phys. Solids 106, 60-79.

\bibitem{holz6} A Pandolfi, GA Holzapfel (2008) Three-dimensional modeling and computational analysis of the human cornea considering distributed collagen fibril orientations Journal of biomechanical engineering 130, 061006.

\bibitem{holz7} N Roxhed, TC Gasser, P Griss, GA Holzapfel, G Stemme (2007) Penetration-enhanced ultrasharp microneedles and prediction on skin interaction for efficient transdermal drug delivery
Journal of Microelectromechanical systems 16, 1429-1440.

\bibitem{holz1} J Stalhand, A Klarbring, GA Holzapfel (2008) Smooth muscle contraction: mechanochemical formulation for homogeneous finite strains
Progress in biophysics and molecular biology 96, 465-481.

\bibitem{deseri3} M.M. Terzi, K. Dayal, L. Deseri, M. Deserno (2015) Revisiting the Link between Lipid Membrane Elasticity and Microscopic Continuum Models, Biophys. J. 108, 87-88.

\bibitem{yuge} Yuge, S., Akiyama, M., Ishii, M., Namkoong, H., Yagi, K., Nakai, Y., Adachi, R., Komatsu, T. (2016) Glycoprotein nanotube traps influenza virus.  Chem. Lett. 2017, 46, 95-97.

\end{thebibliography}


==> virus_chp_Bigoni_ed - Copia/referenc.tex <==
%\clearpage
\begin{thebibliography}{}

\bibitem{bigoni_libro} Bigoni, D. (2012) Nonlinear solid mechanics. Cambridge University Press.

\bibitem{conf1} D. Bigoni, F. Dal Corso, F. Bosi and D. Misseroni (2015) Eshelby-like forces acting on elastic structures: theoretical and experimental proof. Mechanics of Materials, 80, 368-374.

\bibitem{conf4} D. Bigoni, F. Bosi, F. Dal Corso and D. Misseroni (2014) Instability of a penetrating blade. Journal of the Mechanics and Physics of Solids, 64, 411-425

\bibitem{conf2} D. Bigoni, F. Dal Corso, D.Misseroni and F. Bosi (2014) Torsional locomotion. Proceedings of the Royal Society A, 20140599.

\bibitem{conf3} Bosi, F., Misseroni, D., Dal Corso, F. and Bigoni, D. (2015) Self-encapsulation, or the \lq dripping' of an elastic rod. Proceedings of the Royal Society A, 471, 20150195.

\bibitem{boal} Boal, D. (2002) Mechanics of the cell. Cambridge University Press. 

\bibitem{menzel} Daddi-Moussa-Ider, A., Goh, S., Liebchen, B., Hoell, C., Mathijssen, Arnold J.T.M., Guzm\'n-Lastra, F., Scholz, C., Menzel, A.M., L\"owen, H. (2019) Membrane penetration and trapping of an active particle. J. Chem. Phys. 150, 064906. 

\bibitem{deseri1} L. Deseri, P. Pollaci, M. Zingales, K. Dayal (2016) Fractional hereditariness of lipid membranes: instabilities and linearized evolution. J. Mech. Behaviour Biomed. Materials 58, 11-27. 

\bibitem{deseri2} L. Deseri, G. Zurlo (2013) The stretching elasticity of biomembranes determines their line tension and bending rigidity, Biomech. Modeling Mechanobiology 12 1233-1242. 

\bibitem{disher} Discher, D.E., Mohandas, N., Evans E.A. (1994) Molecular maps of red cell deformation: hidden elasticity and in situ connectivity. Science, 266, 1032-1035.

\bibitem{disher2} Discher, D.E., Boal, D.H., Boey, S.K. (1998) Simulations of the erythrocyte cytoskeleton at large deformation - II. micropipette aspiration. Biophys. J.  75, Issue 3, 1584-1597.

\bibitem{eshelby}  Eshelby, J.D. (1951) The force on an elastic singularity. Phil. Trans. Roy. Soc. London A 244, 87-112.

\bibitem{holz4} G Franceschini, D Bigoni, P Regitnig, GA Holzapfel (2006) Brain tissue deforms similarly to filled elastomers and follows consolidation theory J. Mech. Phys. Solids 54, 2592-2620. 


\bibitem{holz2} GA Holzapfel, TC Gasser, RW Ogden (2000) A new constitutive framework for arterial wall mechanics and a comparative study of material models Journal of elasticity and the physical science of solids 61, 1-48. 

\bibitem{holz3} GA Holzapfel, G Sommer, P Regitnig (2004) Anisotropic mechanical properties of tissue components in human atherosclerotic plaques. J. Biomech. Eng. 126, 657-665. 

\bibitem{holz5} LA Mihai, S Budday, GA Holzapfel, E Kuhl, A Goriely (2017) A family of hyperelastic models for human brain tissue J. Mech. Phys. Solids 106, 60-79.

\bibitem{holz6} A Pandolfi, GA Holzapfel (2008) Three-dimensional modeling and computational analysis of the human cornea considering distributed collagen fibril orientations Journal of biomechanical engineering 130, 061006.

\bibitem{holz7} N Roxhed, TC Gasser, P Griss, GA Holzapfel, G Stemme (2007) Penetration-enhanced ultrasharp microneedles and prediction on skin interaction for efficient transdermal drug delivery
Journal of Microelectromechanical systems 16, 1429-1440.

\bibitem{holz1} J Stalhand, A Klarbring, GA Holzapfel (2008) Smooth muscle contraction: mechanochemical formulation for homogeneous finite strains
Progress in biophysics and molecular biology 96, 465-481.

\bibitem{deseri3} M.M. Terzi, K. Dayal, L. Deseri, M. Deserno (2015) Revisiting the Link between Lipid Membrane Elasticity and Microscopic Continuum Models, Biophys. J. 108, 87-88.

\bibitem{yuge} Yuge, S., Akiyama, M., Ishii, M., Namkoong, H., Yagi, K., Nakai, Y., Adachi, R., Komatsu, T. (2016) Glycoprotein nanotube traps influenza virus.  Chem. Lett. 2017, 46, 95-97.

\end{thebibliography}

